PhiZero: A World Model Built Around Physical Language

We introduce PhiZero, a physical world model built around physical language, a compact discrete representation of world-state transitions. Existing physical world models typically predict future videos directly in pixel space, leaving the underlying world dynamics implicit within high-dimensional visual predictors. Motivated by humans' ability to abstract predictive structure from visual experience and organize it in natural language for explicit reasoning, we learn physical language from in-the-wild videos through self-supervision and use it to explicitly reason about how the physical world evolves. Accordingly, PhiZero adopts a reason-then-render paradigm: it first infers future world evolution as a physical-language sequence and then renders the inferred transitions into videos. Extensive experiments across generation and understanding benchmarks validate the ability of PhiZero to model physically coherent world evolution. We further show its potential for realistic and interactive world modeling, fine-grained action-conditioned simulation, and zero-shot motion transfer.

==> output/pdf/motion_language_umap_3d_caption.tex <==
\caption{\textbf{Motion-semantic structure of the learned Pre-FSQ representation.}
Each point denotes a four-second nuScenes clip represented by a 48-dimensional
Pre-FSQ motion feature, standardized per dimension, reduced to 20 principal
components, and embedded with UMAP-3D. The UMAP fit is fully unsupervised;
ego-motion labels are used only for color. The embedding attains 86.1\% 15-NN label
purity and 0.908 trustworthiness. For legibility in a static paper figure, the
the large unoccupied coordinate intervals separating the moving manifold from
the stationary island are compressed with the same label-independent,
piecewise-linear mapping for every point. This display-only transform preserves
the occupied cluster shapes. One isolated straight sample embedded inside the
stationary island is omitted from the visualization only; it remains included
in the sample set and all reported metrics.}


==> output/pdf/robot_motion_umap_post_fsq_3d_caption.tex <==
\caption{\textbf{Post-FSQ robot motion-pattern representations.}
Each point denotes a four-second AGI-Bot clip represented by a 48-dimensional
Post-FSQ motion feature, standardized per dimension, reduced to 20 principal
components, and embedded with UMAP-3D. The embedding is fit without labels;
colors indicate gripper down-close, up-close, down-open, and sweeping motions.
We show the original embedding coordinates from a back view (elevation $20^\circ$, azimuth
$120^\circ$) without sample filtering or coordinate rescaling. The embedding
attains 94.08\% 15-NN label purity and 0.922 trustworthiness.}

